Neural Descriptor Fields: SE(3)-Equivariant Object Representations for Manipulation

We present Neural Descriptor Fields (NDFs), an object representation that encodes both points and relative poses between an object and a target (such as a robot gripper or a rack used for hanging) via category-level descriptors. We employ this representation for object manipulation, where given a task demonstration, we want to repeat the same task on a new object instance from the same category. We propose to achieve this objective by searching (via optimization) for the pose whose descriptor matches that observed in the demonstration. NDFs are conveniently trained in a self-supervised fashion via a 3D auto-encoding task that does not rely on expert-labeled keypoints. Further, NDFs are SE(3)-equivariant, guaranteeing performance that generalizes across all possible 3D object translations and rotations. We demonstrate learning of manipulation tasks from few (5-10) demonstrations both in simulation and on a real robot. Our performance generalizes across both object instances and 6-DoF object poses, and significantly outperforms a recent baseline that relies on 2D descriptors. Project website: https://yilundu.github.io/ndf/.

==> tbl/multiple_category.tex <==
\begin{table}
\footnotesize
\setlength{\tabcolsep}{5.5pt}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|ccc}
    \toprule
    Type & Model & Grasp Success & Place Success & Execution Success \\
     \midrule
    \multirow{3}{*}{Mug} & Dense Object Nets & 0.91 & 0.50 & 0.45 \\
     & Transporter Nets & \\
     & \ours &  0.96 & 0.92 & 0.88 \\ 
     \midrule
    \multirow{3}{*}{Bowl}  & Dense Object Nets &  \\
     & Transporter Nets & \\
     & \ours &  \\
     \midrule
    \multirow{3}{*}{Bottle}  & Dense Object Nets &  \\
     & Transporter Nets & \\
     & \ours &  \\
    \bottomrule
\end{tabular}
} % \resizebox
\caption{\small \textbf{Multi-instance pick-and-place success rates.} }
\label{tbl:multiple_cateogry}
\vspace{-10pt}
\end{table}

% 08/30 AS: harder generalization experiment for multi instance (randomly scaled test objects), DON numbers (without training on as diverse data) - Grasp: 0.88, Place: 0.39, Combined: 0.35
% 08/31 AS: harder generalization experiment for multi instance (randomly scaled test objects), DON numbers (with training on more diverse data) - Grasp: 0.91, Place: 0.50, Combined: 0.45

==> text/limitations.tex <==
\section{Limitations}
%
Several limitations remain.
%
In contrast to Dense Object Nets~\cite{florence2018dense}, the proposed method is currently constrained to \emph{rigid} objects. This issue could be addressed by extending the neural implicit representation by a non-rigid flow field, as has been successfully demonstrated for non-rigid scenes in geometry reconstruction and novel view synthesis~\cite{niemeyer2019occupancy,li2020neural, pumarola2020dnerf,  park2020nerfies, xian2021space, du2021nerflow}.
%
Further, \ourshort{} currently only addresses category-level transfer of \emph{poses} and \emph{points}. Our current approach is not executed closed-loop, and requires an off-the-shelf inverse kinematics and trajectory planning algorithm. It is an exciting area of future work to extend \ourshort{}s to encode full trajectories.
%
Presently, we assume that the place location in the pick-and-place task remains consistent across executions, though in principle...
%
\vsnote{query points?}

==> text/problem_setup.tex <==
\section{Problem Setup and Method Overview}
\label{sec: problem-setup}


\iffalse{
Consider a task where a robot must grasp along the rim of a mug and hang the mug on a rack by its handle. In this task, the system must determine $T_{pick}$ and $T_{place}$, $SE(3)$ poses denoting the end-effector position and orientation before executing the grasp and the placement, respectively. We propose a general-purpose method which enables the system to obtain $T_{pick}$ and $T_{place}$ directly from a segmented point cloud observation of an object whose 3D model and pose is unknown. In particular, given only a small handful of teleoperated demonstrations of the desired pick-and-place behavior as the task specification, our framework produces a semantically/geometrically consistent pick-and-place trajectory which can be executed on objects that were not included in the demonstrations and that are initialized in arbitrary, unseen configurations.

Prior work has addressed this problem in a variety of ways, including through the use of classical pose estimation, supervised keypoint detection and trajectory optimization [kPAM], and behavior cloning in the feature space of a CNN [TransporterNets].

Pose estimation is typically limited to dealing with objects with known 3D models and canonical poses, or requires matching unseen shapes to fixed known templates. kPAM~\cite{manuelli2019kpam} generalizes pose-based pipelines through the use of 3D keypoint detection and trajectory optimization. However, two downsides of their approach are (i) the need to manually specify the semantic keypoints for each task and label them in a dataset, and (ii) the need to set up an explicit optimization problem with costs and constraints that operates on these keypoints and solves for the transformation the robot should apply to the object. If a new task or skill is to be programmed, then new keypoints must be chosen and labeled, and a new optimization problem must be formulated. 

A less tedious/laborious and more intuitive mode of specifying new tasks can be achieved by providing teleoperated demonstrations. For example, consider changing the ``hang a mug on a rack'' task to instead require the robot to grasp the handle and hang the mug by its opening. Ideally, we would be able to directly demonstrate this new desired behavior and have the robot successfully reproduce it. TransporterNets~\cite{zeng2020transporter} moves in this direction by formulating an efficient setup which enables learning pick-and-place behaviors from a small number of demonstrations. Their model is provided with a set of pick-and-place demonstrations, and is trained via behavior cloning to detect pick locations and pick-conditioned place locations (both of which are represented as a pixel location in the image observation). The placement locations are found by cropping the initial image near the pick-pixel and searching for an optimal ``transport'' for the robot to apply. This search is performed by overlaying the dense feature map from the partial crop on another partial crop corresponding to a candidate place pose, and selecting the translation which produces the highest feature correlation between the two crops.

Cruically, TransporterNets makes use of a fully-convolutional network (FCN) which offers 2D translation equivariance, thereby dramatically reducing their data requirements. \asnote{how much of this to explain?}. However, this method only works to obtain a 2D translation action, and the rotational components need to be obtained by a comabination of discretizing + classifying and directly regressing the remaining degrees of freedom. Furthermore, their extensions to enable $SE(3)$ placing do not readily extend to also enable $SE(3)$ grasping. \asnote{is this true?}. Instead we propose a principled method to directly obtain a full $SE(3) $ pose, including both 3D translational and rotational degrees of freedom. 

State space - poses, unknown
Observation space - segmented point cloud from calibrated depth cameras
Action space - collision free arm motion from some initial start pose to some specified goal pose, represented as a relative $SE(3)$ transformation.
}\fi

==> text/todo.tex <==
\pa{
\begin{itemize}
    \item Baseline comparison where we transfer 2D keypoints across object instances. 
\end{itemize}
}
